Non-sparse Linear Representations for Visual Tracking with Online Reservoir Metric Learning

Most sparse linear representation-based trackers need to solve a computationally expensive L1-regularized optimization problem. To address this problem, we propose a visual tracker based on non-sparse linear representations, which admit an efficient closed-form solution without sacrificing accuracy. Moreover, in order to capture the correlation information between different feature dimensions, we learn a Mahalanobis distance metric in an online fashion and incorporate the learned metric into the optimization problem for obtaining the linear representation. We show that online metric learning using proximity comparison significantly improves the robustness of the tracking, especially on those sequences exhibiting drastic appearance changes. Furthermore, in order to prevent the unbounded growth in the number of training samples for the metric learning, we design a time-weighted reservoir sampling method to maintain and update limited-sized foreground and background sample buffers for balancing sample diversity and adaptability. Experimental results on challenging videos demonstrate the effectiveness and robustness of the proposed tracker.

==> ref.bib.0 <==
% BibTeX bibliography file


@STRING{ACCV = {Proc. Asian Conf. Comp. Vis.}}

@STRING{CVIU = {Comp. Vis. Image Understanding}}

@STRING{CVPR = {Proc. IEEE Conf. Comp. Vis. Patt. Recogn.}}

@STRING{ECCV = {Proc. Eur. Conf. Comp. Vis.}}

@STRING{BMVC = {Proc. British Machine  Vis. Conf.}}


@STRING{ICCV = {Proc. IEEE Int. Conf. Comp. Vis.}}

@STRING{ICIP = {Proc. IEEE Int. Conf. Image Process.}}

@STRING{ICML = {Proc. Int. Conf. Mach. Learn.}}

@STRING{IJCAI = {Proc. Int. Joint Conf. Artificial Intell.}}

@STRING{IEEE_J_CASVT = {{IEEE} Trans. Circuits Syst. Video Technol.}}

@STRING{IEEE_J_PAMI = {{IEEE} Trans. Pattern Anal. Mach. Intell.}}

@STRING{IEEE_J_TIP = {{IEEE} Trans. Image Proc.}}

@STRING{IJCV = {Int. J. Comp. Vis.}}

@STRING{JMLR = {J. Mach. Learn. Res.}}

@STRING{ML = {Mach. Learn.}}

@STRING{MS = {Management Sci.}}

@STRING{NIPS = {Proc. Adv. Neural Inf. Process. Syst.}}

@STRING{PR = {Pattern Recogn.}}

@STRING{KDD = {Proc. ACM SIGKDD Int. Conf. Knowledge discovery \& data mining}}




@InProceedings{Adam-Fragment-2006,
  author = {A. Adam and E. Rivlin and I. Shimshoni},
  title = {Robust Fragments-Based Tracking Using the Integral Histogram},
  booktitle = CVPR,
  year = {2006},
  pages = {798-805}
}

@InProceedings{Babenko-Yang-Belongie-cvpr2009,
  author = {B. Babenko and M. Yang and S. Belongie},
  title = {Visual Tracking with Online Multiple Instance Learning},
  booktitle =  CVPR,
  year = {2009},
  pages = {983-990}
}

@InProceedings{Dalal-Triggs-CVPR2005,
  author = {N. Dalal and B. Triggs},
  title = {Histograms of Oriented Gradients for Human Detection},
  booktitle =  CVPR,
  year = {2005}
}

@InProceedings{FaceICCV2011,
  author = {L. Zhang and M. Yang and X. Feng},
  title = {Sparse representation or collaborative representation: Which helps
  face recognition?},
  booktitle =  ICCV,
  year = {2011}
}

@InProceedings{Grabner-Grabner-Bischof-BMVC2006,
  author = {H. Grabner and M. Grabner and H. Bischof},
  title = {Real-time Tracking via On-line Boosting},
  booktitle = BMVC,
  year = {2006},
  pages = {47-56}
}

@Article{Kolonko04sequentialreservoir,
  author = {M. Kolonko and D. W\"asch},
  title = {Sequential Reservoir Sampling with a Non-Uniform Distribution},
  journal = {{ACM} Trans.  Math. Software},
  year = {2004},
  volume = {32},
  pages = {257-273}
}

@InProceedings{Kwon-Lee-CVPR2010,
  author = {J. Kwon and K. M. Lee},
  title = {Visual Tracking Decomposition},
  booktitle = CVPR,
  year = {2010},
  pages = {1269-1276}
}

@InProceedings{Li-Shen-Shi-cvpr2011,
  author = {H. Li and C. Shen and Q. Shi},
  title = {Real-Time Visual Tracking With Compressive Sensing},
  booktitle =  CVPR,
  year = {2011}
}

@Article{Limy-Ross17,
  author = {D. A. Ross and J. Lim and R. Lin and M. Yang},
  title = {Incremental Learning for Robust Visual Tracking},
  journal = IJCV,
  year = {2008},
  volume = {77},
  number = {1},
  pages = {125-141}
}

@Article{Meo-Ling-ICCV09,
  author = {X. Mei and H. Ling},
  title = {Robust Visual Tracking and Vehicle Classification via Sparse
  Representation},
  journal = ieee_j_pami,
  year = {2011}
}

@InProceedings{Shi-Eriksson-Hengel-Shen-cvpr2011,
  author = {Q. Shi and A. Eriksson and A. {van den Hengel} and C. Shen},
  title = {Is face recognition really a Compressive Sensing problem?},
  booktitle = CVPR,
  year = {2011}
}

@Article{chechik2010large,
  author = {Chechik, G. and Sharma, V. and Shalit, U. and Bengio, S.},
  title = {Large scale online learning of image similarity through ranking},
  journal = {J. Mach. Learn. Research},
  year = {2010},
  volume = {11},
  pages = {1109-1135}
}

@Article{crammer2006online,
  author = {Crammer, K. and Dekel, O. and Keshet, J. and Shalev-Shwartz, S. and
  Singer, Y.},
  title = {Online passive-aggressive algorithms},
  journal = {J. Mach. Learn. Research},
  year = {2006},
  volume = {7},
  pages = {551-585}
}

@Article{efraimidis2006weighted,
  author = {Efraimidis, P. S. and Spirakis, P. G.},
  title = {Weighted random sampling with a reservoir},
  journal = {Information process. letters},
  year = {2006},
  volume = {97},
  number = {5},
  pages = {181-185}
}

@InProceedings{globerson2006metric,
  author = {A. Globerson and S. Roweis},
  title = {Metric learning by collapsing classes},
  booktitle = NIPS,
  year = {2006}
}

@InProceedings{harestruck_iccv2011,
  author = {S. Hare and A. Saffari and P.H.S. Torr},
  title = {Struck: Structured Output Tracking with Kernels},
  booktitle = ICCV,
  year = {2011}
}

@book{householder1964theory,
  author = {A. S. Householder},
  title = {The theory of matrices in numerical analysis},
  year = {1964},
  publisher = {Blaisdell Publishing Co.: New York}
}


@article{Generalized2010Shen,
   author   = {C. Shen and J. Kim and H. Wang},
   title    = {Generalized Kernel-based Visual Tracking},
   journal  = {IEEE Trans. Circuits \& Systems for Video Tech.},   
   volume   = {20},
   number   = {1},
   year     = {2010},
   pages    = {119-130},
}



@inproceedings{Shen2009PSD,
   author    = {C. Shen and J. Kim and L. Wang and A.
       {van den Hengel}},
   title     = {Positive semidefinite metric learning with Boosting},
   booktitle = NIPS,
   year      = {2009},
   pages     = {1651-1659},
   volume    = {},
}


@Book{jennings1992matrix,
  author = {Jennings, A. and McKeown, J.},
  title = {Matrix computation},
  year = {1992},
  publisher = {John Wiley \& Sons Inc.}
}

@InProceedings{jiang2011adaptive,
  author = {N. Jiang and W. Liu and Y. Wu},
  title = {Adaptive and discriminative metric differential tracking},
  booktitle = CVPR,
  year = {2011},
  pages = {1161-1168}
}

@InProceedings{jiang2011tracking,
  author = {N. Jiang and W. Liu and H. Su and Y. Wu},
  title = {Tracking low resolution objects by metric preservation},
  booktitle = CVPR,
  year = {2011},
  pages = {1329-1336}
}

@InProceedings{li2007robust,
  author = {Li, X. and Hu, W. and Zhang, Z. and Zhang, X. and Luo, G.},
  title = {Robust visual tracking based on incremental tensor subspace
  learning},
  booktitle =  ICCV,
  year = {2007},
  pages = {1-8}
}

@Article{li2010robust,
  author = {Li, X. and Hu, W. and Wang, H. and Zhang, Z.},
  title = {Robust object tracking using a spatial pyramid heat kernel
  structural information representation},
  journal = {Neurocomputing},
  year = {2010},
  volume = {73},
  number = {16-18},
  pages = {3179--3190},
  publisher = {Elsevier}
}

@InProceedings{li2011graph,
  author = {Li, X. and Dick, A. and Wang, H. and Shen, C. and {van den
      Hengel},
  A.},
  title = {Graph mode-based contextual kernels for robust {SVM} tracking},
  booktitle =  ICCV,
  year = {2011},
  pages = {1156-1163}
}

@InProceedings{lixi-cvpr2008,
  author = {X. Li and W. Hu and Z. Zhang and X. Zhang and M. Zhu and J. Cheng},
  title = {Visual Tracking Via Incremental Log-Euclidean Riemannian Subspace
  Learning},
  booktitle =  CVPR,
  year = {2008},
  pages = {1-8}
}

@Article{powell1969theorem,
  author = {M. J. D. Powell},
  title = {A theorem on rank one modifications to a matrix and its inverse},
  journal = {The Computer Journal},
  year = {1969},
  volume = {12},
  number = {3},
  pages = {288-290}
}

@InProceedings{rigamonti2011sparse,
  author = {Rigamonti, R. and Brown, M. A. and Lepetit, V.},
  title = {Are Sparse Representations Really Relevant for Image
  Classification?},
  booktitle = CVPR,
  year = {2011},
  pages = {1545-1552}
}

@Article{tsagkatakisonline_csvt,
  author = {G. Tsagkatakis and A. Savakis},
  title = {Online Distance Metric Learning for Object Tracking},
  journal = {IEEE Trans. Circuits \& Systems for Video Tech.},
  year = {2011}
}



@Article{vitter1985random,
  author = {Vitter, J. S.},
  title = {Random sampling with a reservoir},
  journal = {ACM Trans. Math. Software},
  year = {1985},
  volume = {11},
  number = {1},
  pages = {37-57}
}

@Article{wang2010discriminative,
  author = {X. Wang and G. Hua and T. Han},
  title = {Discriminative tracking by metric learning},
  journal = eccv,
  year = {2010},
  pages = {200-214}
}

@InProceedings{weinberger2006distance,
  author = {K.Q. Weinberger and J. Blitzer and L.K. Saul},
  title = {Distance metric learning for large margin nearest neighbor
  classification},
  booktitle = NIPS,
  year = {2006}
}

@InProceedings{zhaoICML2011,
  author = {P. Zhao and S.C.H. Hoi and R. Jin and T. Yang},
  title = {Online {AUC} Maximization},
  booktitle = icml,
  year = {2011}
}


